Multivariable control of modular multilevel converters with convergence and safety guarantees

Well-designed current control is a key factor in ensuring the efficient and safe operation of modular multilevel converters (MMCs). Even though this control problem involves multiple control objectives, conventional current control schemes are comprised of independently designed decoupled controllers, e.g., proportional-integral (PI) or proportional-resonant (PR). Due to the bilinearity of the MMC dynamics, tuning PI and PR controllers so that good performance and constraint satisfaction are guaranteed is quite challenging. This challenge becomes more relevant in an AC/AC MMC configuration due to the complexity of tracking the single-phase sinusoidal components of the MMC output. In this paper, we propose a method to design a multivariable controller, i.e., a static feedback gain, to regulate the MMC currents. We use a physics-informed transformation to model the MMC dynamics linearly and synthesise the proposed controller. We use this linear model to formulate a linear matrix inequality that computes a feedback gain that guarantees safe and effective operation, including (i) limited tracking error, (ii) stability, and (iii) meeting all constraints. To test the efficacy of our method, we examine its performance in a direct AC/AC MMC simulated in Simulink/PLECS and in a scaled-down AC/AC MMC prototype to investigate the ultra-fast charging of electric vehicles.

==> bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> bibliography/mybibfileDOI.tex <==
@ARTICLE{IEEE_STD_2010,
  author={IEEE},
  journal={IEEE Std 1459-2010 (Revision of IEEE Std 1459-2000)}, 
  title={IEEE Standard Definitions for the Measurement of Electric Power Quantities Under Sinusoidal, Nonsinusoidal, Balanced, or Unbalanced Conditions}, 
  year={2010},
  volume={},
  number={},
  pages={1-50},
  doi={10.1109/IEEESTD.2010.5439063}}
@ARTICLE{Farias2020MMCSTATCOM,
  author={Farias, João Victor Matos and Cupertino, Allan Fagner and Ferreira, Victor de Nazareth and Pereira, Heverton Augusto and Seleme, Seleme Isaac and Teodorescu, Remus},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Reliability-Oriented Design of Modular Multilevel Converters for Medium-Voltage STATCOM}, 
  year={2020},
  volume={67},
  number={8},
  pages={6206-6214},
  doi={10.1109/TIE.2019.2937050}}
@article{DELAPENA2008ISS,
title = {Design of ISS-Lyapunov Functions for Discrete-Time Linear Uncertain Systems},
journal = {IFAC Proceedings Volumes},
volume = {41},
number = {2},
pages = {1135-1140},
year = {2008},
note = {17th IFAC World Congress},
issn = {1474-6670},
doi = {https://doi.org/10.3182/20080706-5-KR-1001.00196},
author = {D. Muñoz {de la Peña} and T. Alamo and M. Lazar and W.P.M.H. Heemels},
keywords = {Robust control, Robust controller synthesis, LMI optimization based controller synthesis},
abstract = {In this work we consider robust control of discrete-time linear systems affected by time-varying additive disturbance inputs. We present a linear matrix inequality (LMI) based design technique that takes into account in an explicit manner, by means of a Minkowski function, the shape of the set in which the disturbances are bounded. This technique allows one to obtain tight bounds on the performance of the closed-loop system.}
}

@ARTICLE{Perez2021MMCSurvey,
  author={Perez, Marcelo A. and Ceballos, Salvador and Konstantinou, Georgios and Pou, Josep and Aguilera, Ricardo P.},
  journal={IEEE Open Journal of the Industrial Electronics Society}, 
  title={Modular Multilevel Converters: Recent Achievements and Challenges}, 
  year={2021},
  volume={2},
  number={},
  pages={224-239},
  doi={10.1109/OJIES.2021.3060791}}

@article{Challa2023MMCSurvey,
  title={Modeling, Controlling Approaches, Modulation Schemes, and Applications of Modular Multilevel Converter},
  author={Challa, Raghu Vamsi Krishna and Mikkili, Suresh and Bonthagorla, Praveen Kumar},
  journal={Journal of Control, Automation and Electrical Systems},
  volume={34},
  number={1},
  pages={189--215},
  year={2023},
  publisher={Springer}
}

@book{Sharifabadi2016MMCBook,
   author = {Kamran Sharifabadi and Lennart Harnefors and Hans Peter Nee and Staffan Norrga and Remus Teodorescu},
   city = {Chichester, West Sussex, United Kingdom},
   edition = {1},
   isbn = {9781118851562},
   publisher = {John Wiley and Sons, Inc.},
   title = {Design, control and application of modular multilevel converters for HVDC transmission systems},
   year = {2016},
}

@book{Geyer2017MMCBook,
   abstract = {In this original book on model predictive control (MPC) for power electronics, the focus is put on high-power applications with multilevel converters operating at switching frequencies well below 1 kHz, such as medium-voltage drives and modular multi-level converters. Consisting of two main parts, the first offers a detailed review of three-phase power electronics, electrical machines, carrier-based pulse width modulation, optimized pulse patterns, state-of-the art converter control methods and the principle of MPC. The second part is an in-depth treatment of MPC methods that fully exploit the performance potential of high-power converters. These control methods combine the fast control responses of deadbeat control with the optimal steady-state performance of optimized pulse patterns by resolving the antagonism between the two.  },
   author = {Tobias Geyer},
   isbn = {978-1-119-01090-6},
   issn = {978-1-5231-1478-8},
   publisher = {John Wiley and Sons},
   title = {Model Predictive Control of High Power Converters and Industrial Drives },
   year = {2017},
}

@book{Du2018MMCBook,
   author = {Sixing Du and Apparao Dekka and Bin Wu and Navid R. Zargari},
   city = {New Jersey},
   editor = {Tariq Samad},
   isbn = {978-1-119-36630-0},
   keywords = {modular multilevel converter (MMC)},
   pages = {368},
   publisher = {John Wiley and Sons},
   title = {Modular Multilevel Converter: Analysis, Control and Applications},
   year = {2018},
}

@article{Dekka2019MMCSurvey,
   abstract = {Model predictive control (MPC) has emerged as a promising approach to control a modular multilevel converter (MMC). With the help of a cost function, the control objectives of an MMC are achieved easily by using an MPC approach. However, the MPC has several technical challenges and issues including the need of accurate system models, computational complexity, and variable switching frequency operation and weighting factor selection, when it comes to the control of an MMC. In the past few years, several research studies are conducted to address some of the challenges and issues in an MPC and developed several model predictive algorithms for an MMC. In this paper, the importance of each challenge and its impact on the system performance is discussed. Also, the MMC mathematical models used in the implementation of MPC are presented. Furthermore, some of the popular MPC algorithms are discussed briefly, and their features and performance are highlighted through case studies. Finally, summary and future trends of MPC for an MMC are presented.},
   author = {Apparao Dekka and Bin Wu and Venkata Yaramasu and Ricardo Lizana Fuentes and Navid R. Zargari},
   doi = {10.1109/JESTPE.2018.2880137},
   issn = {2168-6777},
   issue = {1},
   journal = {IEEE Journal of Emerging and Selected Topics in Power Electronics},
   keywords = {Capacitor voltage control,circulating current (CC),common-mode voltage (CMV),dc-link current ripple,model predictive control (MPC),modular multilevel converter (MMC)},
   month = {3},
   pages = {168-183},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Model Predictive Control of High-Power Modular Multilevel Converters—An Overview},
   volume = {7},
   year = {2019},
}

@ARTICLE{Sun2022MMCRobust,
  author={Sun, Yuanxiang and Zhang, Zhenbin and Wang, Yongdu and Li, Zhen and Rodriguez, Jose},
  journal={IEEE Transactions on Power Delivery}, 
  title={Robust Predictive Control of Grid-Tied Modular Multilevel Converters for HVDC Systems With Virtual-Flux Based Online Inductance Estimation}, 
  year={2022},
  volume={37},
  number={4},
  pages={3189-3199},
  doi={10.1109/TPWRD.2021.3125036}}

@ARTICLE{Shotorbani2018MMCRobust,
  author={Shotorbani, Amin Mohammadpour and Meng, Xuekun and Wang, Liwei and Mohammadi-Ivatloo, Behnam},
  journal={IEEE Transactions on Industrial Informatics}, 
  title={A Decentralized Multiloop Scheme for Robust Control of a Power Flow Controller With Two Shunt Modular Multilevel Converters}, 
  year={2018},
  volume={14},
  number={10},
  pages={4309-4321},
  doi={10.1109/TII.2018.2799139}}

@ARTICLE{Tavakoli2022MMCRobust,
  author={Tavakoli, Saman Dadjo and Fekriasl, Sajjad and Prieto-Araujo, Eduardo and Beerten, Jef and Gomis-Bellmunt, Oriol},
  journal={IEEE Transactions on Power Delivery}, 
  title={Optimal $\mathcal {H}_{\infty }$ Control Design for MMC-Based HVDC Links}, 
  year={2022},
  volume={37},
  number={2},
  pages={786-797},
  doi={10.1109/TPWRD.2021.3071211}}

@ARTICLE{Zama2021MMCRobust,
  author={Zama, Ahmed and Benchaib, Abdelkrim and Bacha, Seddik and Frey, David and Silvant, Sebastien and Georges, Didier},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Linear Feedback Dead-Beat Control for Modular Multilevel Converters: Validation Under Faults Grid Operation Mode}, 
  year={2021},
  volume={68},
  number={4},
  pages={3181-3191},
  doi={10.1109/TIE.2020.2978708}}

@ARTICLE{Belhaouane2019MMCRobust,
  author={Belhaouane, Mohamed Moez and Ayari, Mohamed and Guillaud, Xavier and Braiek, Naceur Benhadj},
  journal={IEEE Transactions on Industry Applications}, 
  title={Robust Control Design of MMC-HVDC Systems Using Multivariable Optimal Guaranteed Cost Approach}, 
  year={2019},
  volume={55},
  number={3},
  pages={2952-2963},
  doi={10.1109/TIA.2019.2900606}}

@ARTICLE{Böcker2015MMC,
  author={Böcker, Jan and Freudenberg, Benjamin and The, Andrew and Dieckerhoff, Sibylle},
  journal={IEEE Transactions on Power Electronics}, 
  title={Experimental Comparison of Model Predictive Control and Cascaded Control of the Modular Multilevel Converter}, 
  year={2015},
  volume={30},
  number={1},
  pages={422-430},
  doi={10.1109/TPEL.2014.2309438}}

@article{Francis1976LOT,
title = {The internal model principle of control theory},
journal = {Automatica},
volume = {12},
number = {5},
pages = {457-465},
year = {1976},
issn = {0005-1098},
doi = {https://doi.org/10.1016/0005-1098(76)90006-6},
author = {B.A. Francis and W.M. Wonham},
abstract = {Abstract
The classical regulator problem is posed in the context of linear, time-invariant, finite-dimensional systems with deterministic disturbance and reference signals. Control action is generated by a compensator which is required to provide closed loop stability and output regulation in the face of small variations in certain system parameters. It is shown, using the geometric approach, that such a structurally stable synthesis must utilize feedback of the regulated variable, and incorporate in the feedback path a suitably reduplicated model of the dynamic structure of the disturbance and reference signals. The necessity of this control structure constitutes the Internal Model Principle. It is shown that, in the frequency domain, the purpose of the internal model is to supply closed loop transmission zeros which cancel the unstable poles of the disturbance and reference signals. Finally, the Internal Model Principle is extended to weakly nonlinear systems subjected to step disturbances and reference signals.}
}

@article{Francis1977LOT,
author = {Francis, Bruce A.},
title = {The Linear Multivariable Regulator Problem},
journal = {SIAM Journal on Control and Optimization},
volume = {15},
number = {3},
pages = {486-505},
year = {1977},
doi = {10.1137/0315033},
abstract = { The problem is considered of regulating in the face of parameter uncertainty the output of a linear time-invariant system subjected to disturbance and reference signals. This problem has been solved by other researchers. In this paper, a new and simpler algebraic solution is given. }
}
@book{Huang2004NLOT,
  title={Nonlinear output regulation: theory and applications},
  author={Huang, Jie},
  year={2004},
  publisher={SIAM}
}

@ARTICLE{Harnefors2013MMC1,
  author={Harnefors, Lennart and Antonopoulos, Antonios and Norrga, Staffan and Angquist, Lennart and Nee, Hans-Peter},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Dynamic Analysis of Modular Multilevel Converters}, 
  year={2013},
  volume={60},
  number={7},
  pages={2526-2537},
  doi={10.1109/TIE.2012.2194974}}

@INPROCEEDINGS{Antonopoulos2009MMC14,
  author={Antonopoulos, Antonios and Angquist, Lennart and Nee, Hans-Peter},
  booktitle={2009 13th European Conference on Power Electronics and Applications}, 
  title={On dynamics and voltage control of the Modular Multilevel Converter}, 
  year={2009},
  volume={},
  number={},
  pages={1-10},
  doi={}}

@ARTICLE{Angquist2011MMC15,
  author={Angquist, Lennart and Antonopoulos, Antonios and Siemaszko, Daniel and Ilves, Kalle and Vasiladiotis, Michail and Nee, Hans-Peter},
  journal={IEEE Transactions on Industry Applications}, 
  title={Open-Loop Control of Modular Multilevel Converters Using Estimation of Stored Energy}, 
  year={2011},
  volume={47},
  number={6},
  pages={2516-2524},
  doi={10.1109/TIA.2011.2168593}}

@ARTICLE{Antonopoulos2014MMC16,
  author={Antonopoulos, Antonios and Ängquist, Lennart and Harnefors, Lennart and Ilves, Kalle and Nee, Hans-Peter},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Global Asymptotic Stability of Modular Multilevel Converters}, 
  year={2014},
  volume={61},
  number={2},
  pages={603-612},
  doi={10.1109/TIE.2013.2254100}}

@ARTICLE{Harnefors2015MMC17,
  author={Harnefors, Lennart and Antonopoulos, Antonios and Ilves, Kalle and Nee, Hans-Peter},
  journal={IEEE Transactions on Power Electronics}, 
  title={Global Asymptotic Stability of Current-Controlled Modular Multilevel Converters}, 
  year={2015},
  volume={30},
  number={1},
  pages={249-258},
  doi={10.1109/TPEL.2014.2298560}}

@inproceedings{Pereira2023ExampleACAC,
title = "Capacitor voltage ripple and capacitance evaluation in a direct three-phase to single-phase ac/ac MMC",
abstract = "This paper introduces the capacitor current and voltage ripple evaluation of a direct three-phase to single-phase ac/ac modular multilevel converter with full-bridge sub-modules. Based on a desired sub-module capacitor voltage ripple, the required capacitance is calculated, which is valuable to dimension sub-modules{\textquoteright} energy storage in many applications. Simulations and measurements using a scaled-down prototype validate the analysis.",
keywords = "Battery, Capacitance, Capacitor RMS current, Capacitor voltage ripple, Full-bridge, Medium-voltage, MMC",
author = "{Pereira Marca}, Ygor and Roes, {Maurice G.L.} and Wijnands, {Korneel G.E.}",
year = "2023",
month = may,
day = "24",
language = "English",
booktitle = "11th International Conference on Power Electronics, ICPE 2023 ECCE Asia",
publisher = "Institute of Electrical and Electronics Engineers",
address = "United States",
note = "11th International Conference on Power Electronics - ECCE Asia, ICPE 2023 ECCE Asia ; Conference date: 22-05-2023 Through 25-05-2023",
}

@inproceedings{Pereira2022ExampleACSquare,
title = "Square wave operation to reduce pulsating power in isolated MMC-based ultrafast chargers",
abstract = "This paper presents an application of modular multilevel converters to reduce pulsating power, and therefore sub-modules in ultrafast chargers. The converter{\textquoteright}s analysis and a control scheme were presented to realize bidirectional power transfer between a three-phase medium-voltage grid and a single-phase medium-frequency transformer with square-shaped voltage, successfully reducing power fluctuation.",
keywords = "Charger, Full-bridge sub-modules, Medium-frequency transformer, Medium-voltage grid, Modular multilevel converter (MMC), Square wave, Modular multilevel converter",
author = "{Pereira Marca}, Ygor and Roes, {Maurice G.L.} and Duarte, {Jorge L.} and C.G.E. Wijnands",
year = "2022",
month = oct,
day = "17",
language = "English",
booktitle = "24th European Conference on Power Electronics and Applications, EPE 2022 ECCE Europe",
publisher = "Institute of Electrical and Electronics Engineers",
address = "United States",
note = "24th European Conference on Power Electronics and Applications, EPE 2022 ECCE Europe, EPE'22 ECCE Europe ; Conference date: 05-09-2022 Through 09-09-2022",
}

@inproceedings{Pereira2021ExampleACDC,
title = "Extended operating region of modular multilevel converters using full-bridge sub-modules",
abstract = "This paper presents an application of modular multilevel converters to remove line-frequency transformers from ultrafast charging stations, reducing cost and volume. The converter analysis with full-bridge sub-modules enables an operating region, that converts a medium-voltage grid into a lower voltage DC-bus, ideal for charging batteries rapidly.",
keywords = "battery, charger, Full-bridge, Medium-voltage grid, modular multilevel converter, Battery, Modular multilevel converter, Charger",
author = "{Pereira Marca}, Ygor and Duarte, {Jorge L.} and Roes, {Maurice G.L.} and Wijnands, {C.G.E. (Korneel)}",
year = "2021",
month = oct,
day = "25",
language = "English",
booktitle = "2021 23rd European Conference on Power Electronics and Applications (EPE'21 ECCE Europe)",
publisher = "Institute of Electrical and Electronics Engineers",
address = "United States",
note = "23rd European Conference on Power Electronics and Applications, EPE 2021 ECCE Europe, EPE 2021 ; Conference date: 06-09-2021 Through 10-09-2021",
}

@inproceedings{Pereira2021ExampleACAC,
title = "Isolated MMC-based ac/ac stage for ultrafast chargers",
abstract = "The application of indirect and direct modular multilevel converter-based topologies in an isolated ultrafast charger, operating from a three-phase medium-voltage grid, is compared. The most promising circuit is an isolated direct ac/ac modular multilevel converter, in which four-quadrant operation is possible by employing full-bridge sub-modules. The direct ac/ac conversion reduces the cost and volume of fast charging stations by eliminating line frequency transformers. An analytical model focusing on the decomposition of circuit states is employed to present the control scheme. Subsequently, the approach is validated with simulation results, corroborating the suitability for high-power bidirectional battery chargers.",
keywords = "battery, full-bridge, isolated, medium-voltage, modular multilevel converter, transformer, ultrafast charger",
author = "{Pereira Marca}, Ygor and Roes, {Maurice G.L.} and Duarte, {Jorge L.} and Wijnands, {C.G.E. (Korneel)}",
year = "2021",
month = nov,
day = "13",
doi = "10.1109/ISIE45552.2021.9576217",
language = "English",
booktitle = "2021 IEEE 30th International Symposium on Industrial Electronics (ISIE)",
publisher = "Institute of Electrical and Electronics Engineers",
address = "United States",
note = "30th International Symposium on Industrial Electronics: Full Online Conference, IESIE 2021 ; Conference date: 20-06-2021 Through 23-06-2021",
}

@ARTICLE{Marquardt2018MMCSurvey,
  author={Marquardt, Rainer},
  journal={IEEE Power Electronics Magazine}, 
  title={Modular Multilevel Converters: State of the Art and Future Progress}, 
  year={2018},
  volume={5},
  number={4},
  pages={24-31},
  doi={10.1109/MPEL.2018.2873496}}

@INPROCEEDINGS{Marquardt2003MMC,
  author={Lesnicar, A. and Marquardt, R.},
  booktitle={2003 IEEE Bologna Power Tech Conference Proceedings,}, 
  title={An innovative modular multilevel converter topology suitable for a wide power range}, 
  year={2003},
  volume={3},
  number={},
  pages={6 pp. Vol.3-},
  doi={10.1109/PTC.2003.1304403}}


@INPROCEEDINGS{Darivianakis2014MMCMPCSurvey,
  author={Darivianakis, Georgios and Geyer, Tobias and van der Merwe, Wim},
  booktitle={2014 IEEE Energy Conversion Congress and Exposition (ECCE)}, 
  title={Model predictive current control of modular multilevel converters}, 
  year={2014},
  volume={},
  number={},
  pages={5016-5023},
  doi={10.1109/ECCE.2014.6954089}}

@ARTICLE{Aguilera2017MMC,
  author={Aguilera, Ricardo P. and Acuña, Pablo and Lezana, Pablo and Konstantinou, Georgios and Wu, Bin and Bernet, Steffen and Agelidis, Vassilios G.},
  journal={IEEE Transactions on Power Electronics}, 
  title={Selective Harmonic Elimination Model Predictive Control for Multilevel Power Converters}, 
  year={2017},
  volume={32},
  number={3},
  pages={2416-2426},
  doi={10.1109/TPEL.2016.2568211}}

@INPROCEEDINGS{Lopez2014MMC,
  author={Lopez, Andres and Quevedo, Daniel E. and Aguilera, Ricardo and Geyer, Tobias and Oikonomou, Nikolaos},
  booktitle={2014 4th Australian Control Conference (AUCC)}, 
  title={Reference design for predictive control of modular multilevel converters}, 
  year={2014},
  volume={},
  number={},
  pages={239-244},
  doi={10.1109/AUCC.2014.7358697}}

@INPROCEEDINGS{Rohner2011MMCModelling,
  author={Rohner, Steffen and Weber, Jens and Bernet, Steffen},
  booktitle={2011 IEEE Energy Conversion Congress and Exposition}, 
  title={Continuous model of Modular Multilevel Converter with experimental verification}, 
  year={2011},
  volume={},
  number={},
  pages={4021-4028},
  doi={10.1109/ECCE.2011.6064316}}

@INPROCEEDINGS{Song2018MMCACAC,
  author={SONG, Shuguang and LIU, Jinjun and OUYANG, Shaodi and CHEN, Xingxing and LIU, Baojin},
  booktitle={2018 International Power Electronics Conference (IPEC-Niigata 2018 -ECCE Asia)}, 
  title={Control of Direct AC/AC Modular Multilevel Converter in Railway Power Supply System}, 
  year={2018},
  volume={},
  number={},
  pages={1051-1055},
  doi={10.23919/IPEC.2018.8508001}}

@PHDTHESIS{Fuchs2022MMCPhD,
	copyright = {In Copyright - Non-Commercial Use Permitted},
	year = {2022},
	type = {Doctoral Thesis},
	author = {Fuchs, Simon},
	size = {313 p.},
	keywords = {Modular multilevel converter (MMC, M2C); Model predictive control (MPC); optimization; PWM; Rectifier systems; Optimal control},
	language = {en},
	address = {Zurich},
	publisher = {ETH Zurich},
	DOI = {10.3929/ethz-b-000558253},
	title = {MMCs Made Compact and Fast - Towards Modular Multilevel Converters with Minimized Module Capacitors and Fast Transient Operation Utilizing Advanced Control Methods},
	school = {ETH Zurich}
}
@article{YU2023MMCACAC,
title = {Control method of an AC-AC MMC for open-end stator winding wind turbine generation system},
journal = {International Journal of Electrical Power and Energy Systems},
volume = {153},
pages = {109268},
year = {2023},
issn = {0142-0615},
doi = {https://doi.org/10.1016/j.ijepes.2023.109268},
url = {https://www.sciencedirect.com/science/article/pii/S0142061523003253},
author = {Jiali Yu and Xiaoxin Hou and Chaoying Xia and Guodong You and Zhifeng Liu},
keywords = {Modular multi-level converter, Direct ac-ac converter, Wind power generation system, Open-end stator winding permanent magnet synchronous generator, Unified capacitor voltage balance control},
abstract = {With the increasing of power rating and voltage level of wind turbine, the traditaional low voltage converter is being replaced by multilevel converter. This paper proposes a new ac-ac modular multi-level converter (MMC) connecting the open-end stator winding permanent magnet synchronous generator (OW-PMSG) to AC power grid. The working principle of the proposed topology is analyzed. Under different grid conditions, a unified capacitor voltage balance control method and a current control method are proposed. Aiming at the low grid voltage ride through problem, a distributed braking chopper circuit and the corresponding control strategy is given. Simulation is conducted for verification. Compared with the back to back (BTB) MMC for OW-PMSG, the number of capacitors and arm inductors of the proposed topology are reduced by 43% and 33%. Moreover, the number of the state variables of the average capacitor voltages and currents of the proposed topology are reduced by 33% and 47%, reducing the control complexity. The proposed topology also has higher efficiency than the BTB MMC for OW-PMSG. Compared with the other ac-ac MMC topologies for OW-PMSG, the combined power rating of the power devices of the proposed topology is much lower and thus the proposed topology has higher power density.}
}
@article{Meng2020MMCACAC,
author = {Meng, Yongqing and Yu, Jianyang and Shang, Shuonan and Liu, Bo and Gao, Xin},
title = {Modeling and Control of Modular Multilevel AC/AC Converter in Y Configuration for Fractional Frequency Transmission System},
journal = {IEEJ Transactions on Electrical and Electronic Engineering},
volume = {15},
number = {5},
pages = {741-750},
keywords = {Y-MMC, low frequency power transmission and distribution systems, FFTS, mathematical model, control strategy},
doi = {https://doi.org/10.1002/tee.23110},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/tee.23110},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/tee.23110},
abstract = {The modular multilevel AC/AC converter topology in Y configuration, which is called Y-MMC, suitable for fractional frequency transmission system is proposed in this paper. Y-MMC can directly connect two three-phase AC systems of different frequencies and voltage amplitudes with only six equivalent branches, and it has satisfying performance in power quality and characteristics. Y-MMC enjoys a simple and symmetrical structure with no circulating current problem. The detailed topology and operating principle of Y-MMC are addressed in this paper. The frequency-decoupled mathematical model of the Y-MMC system is deduced. Corresponding control scheme is thoroughly designed, including the inner loop current control, the outer loop control, the individual-balancing control, and frequency leakage suppression control. The paper also lays emphasis on the optimization of reactive power distribution between the main branches and the assistant branches of Y-MMC. The validity of the Y-MMC topology and the effectiveness of the proposed control scheme are verified by the simulation results in MATLAB/Simulink. © 2020 Institute of Electrical Engineers of Japan. Published by John Wiley \and Sons, Inc.},
year = {2020}
}
@article{YU2022MMCACAC,
title = {Operation and control schemes of a novel direct AC-AC modular multilevel converter},
journal = {International Journal of Electrical Power and Energy Systems},
volume = {139},
pages = {108037},
year = {2022},
issn = {0142-0615},
doi = {https://doi.org/10.1016/j.ijepes.2022.108037},
url = {https://www.sciencedirect.com/science/article/pii/S0142061522000801},
author = {Jiali Yu and Chaoying Xia},
keywords = {A novel direct AC-AC MMC topology, Capacitor voltage fluctuation, Common-mode voltage, Current stress},
abstract = {AC-DC-AC modular multilevel converter (MMC) and direct AC-AC MMC are two kinds of interfaces to integrating AC motors into power grid, and they are easily damaged from large capacitor voltage fluctuation with varying motor speed. Up to now, none of the methods could balance the reliability and power density of MMC-based motor drives system. To find a better solution to this problem, a novel direct AC-AC MMC topology is proposed in this paper. Operating principle of this topology is introduced and relative multi-loop feedback control method is designed for it. Then, simulation and experiments are conducted for verification. Compared with the traditional MMC with high-frequency injection method, the proposed topology has no common-mode voltage problem and the current stress is reduced by 38.5%. Compared with the half-bridge-based AC-DC-AC MMC, the number of capacitors and inductors of the proposed topology is reduced by 20.8% and 25%. In comparison with the direct AC-AC MMC (modular multilevel matrix converter), the number of power devices of the proposed topology is reduced by 28%. The proposed topology has higher reliability and power density.}
}

@Article{Gontijo2020MMCACAC,
AUTHOR = {Gontijo, Gustavo and Wang, Songda and Kerekes, Tamas and Teodorescu, Remus},
TITLE = {New AC–AC Modular Multilevel Converter Solution for Medium-Voltage Machine-Drive Applications: Modular Multilevel Series Converter},
JOURNAL = {Energies},
VOLUME = {13},
YEAR = {2020},
NUMBER = {14},
ARTICLE-NUMBER = {3664},
URL = {https://www.mdpi.com/1996-1073/13/14/3664},
ISSN = {1996-1073},
ABSTRACT = {Due to its scalability, reliability, high power quality and flexibility, the modular multilevel converter is the standard solution for high-power high-voltage applications in which an AC-DC-AC connection is required such as high-voltage direct-current transmission systems. However, this converter presents some undesired features from both structural and operational perspectives. For example, it presents a high number of components, which results in high costs, size, weight and conduction losses. Moreover, the modular multilevel converter presents problems dealing with DC-side faults, with unbalanced grid conditions, and many internal control loops are required for its proper operation. In variable-frequency operation, the modular multilevel converter presents some serious limitations. The most critical are the high-voltage ripples, in the submodule capacitors, at low frequencies. Thus, many different AC-DC-AC converter solutions, with modular multilevel structure, have been proposed as alternatives for high-power machine-drive applications such as offshore wind turbines, pumped-hydro-storage systems and industrial motor drives. These converters present their own drawbacks mostly related to control complexity, operational limitations, size and weight. This paper introduces an entirely new medium-voltage AC-DC-AC modular multilevel converter solution with many operational and structural advantages in comparison to the modular multilevel converter and other alternative topologies. The proposed converter presents high performance at low frequencies, regarding the amplitude of the voltage ripples in the submodule capacitors, which could make it very suitable for machine-drive applications. In this paper, an analytical description of the voltage ripples in the submodule capacitors is proposed, which proves the high performance of the converter under low-frequency operation. Moreover, the proposed converter presents high performance under unbalanced grid conditions. This important feature is demonstrated through simulation results. The converter solution introduced in this paper has a simple structure, with decoupled phases, which leads to the absence of undesired circulating currents and to a straightforward control, with very few internal control loops for its proper operation, and with simple modulation. Since the converter phases are decoupled, no arm inductors are required, which contributes to the weight and size reduction of the topology. In this paper, a detailed comparison analysis with the modular multilevel converter is presented based on number of components, conduction and switching losses. This analysis concludes that the proposed converter solution presents a reduction in costs and an expressive reduction in size and weight, in comparison to the modular multilevel converter. Thus, it should be a promising solution for high-power machine-drive applications that require compactness and lightness such as offshore wind turbines. In this paper, simulation results are presented explaining the behavior of the proposed converter, proving that it is capable of synthesizing a high-power-quality load voltage, with variable frequency, while exchanging power with the grid. Thus, this topology could be used to control the machine speed in a machine-drive application. Finally, experimental results are provided to validate the topology.},
DOI = {10.3390/en13143664}
}
@ARTICLE{meng2022MMCACAC,
  author={Meng, Yongqing and Sun, Jialu and Duan, Ziyue and Jia, Feng and Wang, Xiuli and Wang, Xifan},
  journal={IEEE Journal of Emerging and Selected Topics in Power Electronics}, 
  title={Variable Voltage Variable Frequency Modular Multilevel AC/AC Converter With High-Frequency Harmonics Filtering Capability}, 
  year={2022},
  volume={10},
  number={1},
  pages={811-821},
  doi={10.1109/JESTPE.2021.3091996}}

@inproceedings{Pouresmaeil2022MFT,
title = "Single-Phase Bidirectional ZVZCS AC-DC Converter for MV-Connected Ultra-Fast Chargers",
abstract = "A single-phase bidirectional converter fed by a Modular Multilevel Converter (MMC) through a MediumFrequency Transformer (MFT) is a promising solution for medium-voltage-connected chargers of Electric Vehicles (EV). An operating scheme is developed for the converter to realize Zero-Voltage Switching(ZVS) and nearly Zero-Current Switching (ZCS) over the full load range. In comparison with conventional Phase Shift Control (PSC), the proposed scheme significantly reduces the reactive power through the AC-DC converter, thereby decreasing turn-off switching losses and the RMS current through the outputcapacitor. A trade-off between RMS current stresses and the required minimum number of sub-modules in the MMC side is found and studied to provide insights on how the proposed method affects the overall performance of the system. Simulations results are provided to verify the analytical findings.",
author = "Kaveh Pouresmaeil and Duarte, {Jorge L.} and Wijnands, {C.G.E. (Korneel)} and Roes, {Maurice G.L.} and Baars, {Nico H.}",
year = "2022",
doi = "10.30420/565822020",
language = "English",
pages = "124--130",
booktitle = "PCIM Europe 2022",
publisher = "VDE Verlag",
address = "Germany",
note = "2022 International Exhibition and Conference for Power Electronics, Intelligent Motion (PCIM Europe 2022) ; Conference date: 10-05-2022 Through 12-05-2022",
}
%-------------------------------------------------------------------------------------
%----------------------------------------Types----------------------------------------
%-------------------------------------------------------------------------------------
% article
                %An article from a journal or magazine.
% book
                %A book with an explicit publisher.
% booklet
                %A work that is printed and bound, but without a named publisher or sponsoring institution.
% ceedings
                %An article in a conference proceedings.
% proceedings
                %The proceedings of a conference.
% conference
                %The same as inproceedings.
% inbook
                %A part of a book, which may be a chapter (or section or whatever) and/or a range of pages.
% incollection
                %A part of a book having its own title.
% manual
                %Technical documentation.
% mastersthesis
                %A Master's thesis.
% misc
                %Use this type when nothing else fits.
% phdthesis
                %A PhD thesis.
% techreport
                %A report published by a school or other institution, usually numbered within a series.
% unpublished
                %A document having an author and title, but not formally published.
% collection
                %A collection of works. The same as proceedings
% patent
                %A patent.

%-------------------------------------------------------------------------------------
%----------------------------------------Fields---------------------------------------
%-------------------------------------------------------------------------------------
%address
                %Usually the address of the publisher or other type of institution.
%annote
                %An annotation. It is not used by the standard bibliography styles, but may be used by others that produce an annotated bibliography.
%author
                %The name(s) of the author(s), in the format described in the LaTeX book.
%booktitle
                %Title of a book, part of which is being cited. See the LaTeX book for how to type titles. For book entries, use the title field instead.
%chapter
                %A chapter (or section or whatever) number.
%crossref
                %The database key of the entry being cross referenced. Any fields that are missing from the current record are inherited from the field being cross referenced.
%edition
                %The edition of a book---for example, ``Second''. This should be an ordinal, and should have the first letter capitalized, as shown here; the standard styles convert to lower case when necessary.
%editor
                %Name(s) of editor(s), typed as indicated in the LaTeX book. If there is also an author field, then the editor field gives the editor of the book or collection in which the reference appears.
%howpublished
                %How something strange has been published. The first word should be capitalized.
%institution
                %The sponsoring institution of a technical report.
%journal
                %A journal name. Abbreviations are provided for many journals.
%key
                %Used for alphabetizing, cross referencing, and creating a label when the ``author'' information is missing. This field should not be confused with the key that appears in the cite command and at the beginning of the database entry.
%month
                %The month in which the work was published or, for an unpublished work, in which it was written. You should use the standard three-letter abbreviation, as described in Appendix B.1.3 of the LaTeX book.
%note
                %Any additional information that can help the reader. The first word should be capitalized.
%number
                %The number of a journal, magazine, technical report, or of a work in a series. An issue of a journal or magazine is usually identified by its volume and number; the organization that issues a technical report usually gives it a number; and sometimes books are given numbers in a named series.
%organization
                %The organization that sponsors a conference or that publishes a manual.
%pages
                %One or more page numbers or range of numbers, such as 42--111 or 7,41,73--97 or 43+(the `+' in this last example indicates pages following that don't form a simple range). To make it easier to maintain Scribe-compatible databases, the standard styles convert a single dash (as in 7-33) to the double dash used in TeX to denote number ranges (as in 7--33).
%publisher
                %The publisher's name.
%school
                %The name of the school where a thesis was written.
%series
                %The name of a series or set of books. When citing an entire book, the the title field gives its title and an optional series field gives the name of a series or multi-volume set in which the book is published.
%title
                %The work's title, typed as explained in the LaTeX book.
%type
                %The type of a technical report---for example, ``Research Note''.
%volume
                %The volume of a journal or multi-volume book.
%year
                %The year of publication or, for an unpublished work, the year it was written. Generally it should consist of four numerals, such as 1984, although the standard styles can handle any year whose last four nonpunctuation characters are numerals, such as `\hbox{(about 1984)}'.
%affiliation
                %The authors affiliation.
%abstract
                %An abstract of the work.
%contents
                %A Table of Contents
%copyright
                %Copyright information.
%ISBN
                %The International Standard Book Number.
%ISSN
                %The International Standard Serial Number. Used to identify a journal.
%keywords
                %Key words used for searching or possibly for annotation.
%language
                %The language the document is in.
%location
                %A location associated with the entry, such as the city in which a conference took place.
%LCCN
                %The Library of Congress Call Number. I've also seen this as lib-congress.
%mrnumber
                %The Mathematical Reviews number.
%price
                %The price of the document.
%size
                %The physical dimensions of a work.
%URL
                %The WWW Universal Resource Locator that points to the item being referenced. This often is used for technical reports to point to the ftp site where the postscript source of the report is located.

===============================================================================================================================



